Will the Prince Get True Love's Kiss? On the Model Sensitivity to Gender Perturbation over Fairytale Texts

In this paper, we study whether language models are affected by learned gender stereotypes during the comprehension of stories. Specifically, we investigate how models respond to gender stereotype perturbations through counterfactual data augmentation. Focusing on Question Answering (QA) tasks in fairytales, we modify the FairytaleQA dataset by swapping gendered character information and introducing counterfactual gender stereotypes during training. This allows us to assess model robustness and examine whether learned biases influence story comprehension. Our results show that models exhibit slight performance drops when faced with gender perturbations in the test set, indicating sensitivity to learned stereotypes. However, when fine-tuned on counterfactual training data, models become more robust to anti-stereotypical narratives. Additionally, we conduct a case study demonstrating how incorporating counterfactual anti-stereotype examples can improve inclusivity in downstream applications.

==> extra/bart-original.tex <==
\begin{table}[]
    \scalebox{0.95}{
    \footnotesize
    \begin{tabular}{lcccc}
    \toprule
    \textbf{\begin{tabular}[c]{@{}c@{}}Question\\ Type\end{tabular}} & \textbf{Original} & \textbf{\begin{tabular}[c]{@{}c@{}}Rule-\\ Based\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}LLM\\ Rewrite\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}LLM- \\ Assisted \\ Rule-\\ Based\end{tabular}} \\
    
    \midrule
    
    ALL             & 59.12 & 59.73* & 59.02 & 59.31 \\
    \midrule
    Setting         & 85.49 & 84.30 & 86.60 & 81.83 \\
    
    Character       & 80.58 & 80.42 & 79.01 & 78.72 \\
    
    Action          & 65.17 & 66.68* & 65.91 & 63.96* \\
    
    Outcome Res.    & 57.07 & 60.69 & 57.79 & 53.44 \\
    
    Feeling         & 41.87 & 41.87 & 39.96 & 48.14 \\
    
    Causal Rel.     & 51.77 & 51.24 & 50.86 & 52.57 \\
    
    Prediction      & 32.74 & 34.20 & 35.11 & 38.69\\
    
    \bottomrule
    \end{tabular}
    }
    \small
    \caption{\label{bart-rouge-original}ROUGE-L F1 scores for the BART model fine-tuned on the original \texttt{FairytaleQA}  dataset and tested on each CDA approach.
    * values are statistically significant to the 95\% confidence. }

    \end{table}

==> extra/bart_full.tex <==
\footnotesize
    \scalebox{0.87}{
    \begin{tabular}{lcccc|cccc|cccc}
    \toprule
     & \multicolumn{4}{c}{\textbf{Augmented Data}} & \multicolumn{4}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}50\% Original + \\ 50\% Augmented Data\end{tabular}}} & \multicolumn{4}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Full Original + \\ Full Augmented Data\end{tabular}}} 
     \\
     \cmidrule{2-5}\cmidrule{6-9}\cmidrule{10-13}
    \textbf{\begin{tabular}[c]{@{}l@{}}Question \\ Type\end{tabular}} & \textbf{Orig.} & \textbf{\begin{tabular}[c]{@{}c@{}}Rule- \\ Based\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}LLM\\ Rewrite\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}LLM-\\ Assisted \\ Rule- \\ Based\end{tabular}} & \textbf{Orig.} & \textbf{\begin{tabular}[c]{@{}c@{}}Rule- \\ Based\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}LLM\\ Rewrite\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}LLM- \\ Assisted \\ Rule- \\ Based\end{tabular}} & \textbf{Orig.} & \textbf{\begin{tabular}[c]{@{}c@{}}Rule- \\ Based\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}LLM\\ Rewrite\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}} LLM- \\ Assisted \\ Rule- \\ Based\end{tabular}} \\
    
    \toprule
    
    ALL & \textbf{60.28} & \textbf{59.97} & 58.70 & 59.31 & \textbf{60.40} & 58.97 & 58.88 & \textbf{59.65} & \textbf{60.59} & \textbf{60.68} & 59.20 & \textbf{60.07} \cr
    \midrule
    Setting & 81.85 & 83.55 & 87.03 & 81.83 & 81.67 & 83.80 & 85.12 & 81.83 & 81.53 & 81.21 & 82.85 & 80.64 \cr
    Character & 79.19 & 79.90 & 76.35 & 78.72 & 79.56 & 78.81 & 75.47 & 80.24 & 79.34 & 79.65 & 77.65 & 80.54 \cr
    Action & \textbf{67.19} & 66.96 & 66.08 & 63.96 & \textbf{68.53} & 65.95 & 66.42 & 64.70 & \textbf{68.05} & 67.41 & 66.23 & 66.33 \cr
    Outcome Res. & 56.89 & 56.52 & 53.91 & 53.44 & 55.09 & 52.24 & 58.08 & 58.67 & 59.08 & 59.26 & 61.69 & 57.09 \cr
    Feeling & 47.20 & 45.18 & 41.85 & 48.14 & 42.91 & 41.97 & 40.99 & 45.74 & 41.76 & 45.33 & 40.59 & 46.28 \cr
    Causal Rel. & 51.53 & 51.22 & 50.55 & 52.57 & 52.73 & 51.63 & 50.94 & 51.73 & \textbf{53.47} & \textbf{53.56} & 51.51 & 52.63 \cr
    Prediction & 39.14 & 37.63 & 36.10 & 38.69 & 38.06 & 37.21 & 35.13 & 39.16 & 37.76 & 35.62 & 33.66 & 35.54 \cr
    \bottomrule
    \end{tabular}
    }
    \caption{\label{bart-rouge-full}ROUGE-L F1 scores for the BART model fine-tuned on the ruled-based gender augmented \texttt{FairytaleQA}  dataset (l.h.s.), 50\% of original + 50\% of rule-based gender augmented \texttt{FairytaleQA}  dataset (center), and full original + full rule-based gender augmented \texttt{FairytaleQA}  dataset (r.h.s.) and tested on the rule-based gender augmentation, LLM gender augmentation, and LLM assisted rule based gender augmentation test dataset. Bold values indicate a statistically significant increase to the 95\% confidence compared to the results in Table~\ref{bart-rouge-original}.}

==> extra/t5-original.tex <==
\begin{table}[h]
\centering
\footnotesize
\scalebox{0.93}{
\begin{tabular}{@{}l@{ }cccc@{}}
\toprule
\textbf{\begin{tabular}[c]{@{}c@{}}Question\\ Type\end{tabular}} & \textbf{Original} & \textbf{\begin{tabular}[c]{@{}c@{}}Rule-\\ Based\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}LLM\\ Rewrite\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}} LLM-Assisted \\ Rule-Based\end{tabular}} \\

\midrule

ALL &           65.29  & 64.38*   & 63.53*   & 62.66* \\
\midrule
Setting &       89.61  & 87.87    & 87.92    & 85.25* \\

Character &     85.67  & 83.86    & 79.77*   & 82.10* \\

Action &        74.70  & 74.48    & 72.84*   & 72.08* \\

Outcome Res. &  56.94  & 53.80    & 55.00    & 57.46  \\

Feeling &       49.41  & 48.47    & 47.49    & 43.75  \\

Causal Rel. &   56.98  & 56.40    & 56.64    & 55.29* \\

Prediction &    35.57  & 34.98    & 35.28    & 33.31  \\
\bottomrule   
\end{tabular}
}
\caption{\label{t5-rouge-original}ROUGE-L F1 scores for the T5 model fine-tuned on the original \texttt{FairytaleQA} dataset 
% and tested on the rule-based gender augmentation, LLM gender augmentation, and LLM assisted rule based gender augmentation test dataset.
and tested on each CDA approach.
* values are statistically significant to the 95\% confidence.}
\end{table}

==> extra/t5-simplified.tex <==
\begin{table}[h]
\centering
\footnotesize
\scalebox{0.93}{
\begin{tabular}{@{}l@{ }cccc@{}}
\toprule
\textbf{\begin{tabular}[c]{@{}c@{}}Question\\ Type\end{tabular}} & \textbf{Original} & \textbf{\begin{tabular}[c]{@{}c@{}}Rule-\\ Based\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}LLM\\ Rewrite\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}} LLM-Assisted \\ Rule-Based\end{tabular}} \\

\midrule

ALL &           65.29  & 64.38*   & 63.53*   & 62.66* \\
\midrule
Setting &       89.61  & 87.87    & 87.92    & 85.25* \\

Character &     85.67  & 83.86    & 79.77*   & 82.10* \\

Action &        74.70  & 74.48    & 72.84*   & 72.08* \\

Outcome Res. &  56.94  & 53.80    & 55.00    & 57.46  \\

Feeling &       49.41  & 48.47    & 47.49    & 43.75  \\

Causal Rel. &   56.98  & 56.40    & 56.64    & 55.29* \\

Prediction &    35.57  & 34.98    & 35.28    & 33.31  \\
\bottomrule   
\end{tabular}
}
\caption{\label{t5-rouge-original}ROUGE-L F1 scores for the T5 model fine-tuned on the original \texttt{FairytaleQA} dataset 
% and tested on the rule-based gender augmentation, LLM gender augmentation, and LLM assisted rule based gender augmentation test dataset.
and tested on each CDA approach.
* values are statistically significant to the 95\% confidence.}
\end{table}

==> extra/t5_full.tex <==
\begin{table*}[ht!]
    \footnotesize
    \scalebox{0.87}{
    \begin{tabular}{lcccc|cccc|cccc}
    \toprule
     & \multicolumn{4}{c}{\textbf{Augmented Data}} & \multicolumn{4}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}50\% Original + \\ 50\% Augmented Data\end{tabular}}} & \multicolumn{4}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Full Original + \\ Full Augmented Data\end{tabular}}} 
     \\
     \cmidrule{2-5}\cmidrule{6-9}\cmidrule{10-13}
    \textbf{\begin{tabular}[c]{@{}l@{}}Question \\ Type\end{tabular}} & \textbf{Orig.} & \textbf{\begin{tabular}[c]{@{}c@{}}Rule- \\ Based\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}LLM\\ Rewrite\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}LLM-\\ Assisted \\ Rule- \\ Based\end{tabular}} & \textbf{Orig.} & \textbf{\begin{tabular}[c]{@{}c@{}}Rule- \\ Based\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}LLM\\ Rewrite\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}LLM- \\ Assisted \\ Rule- \\ Based\end{tabular}} & \textbf{Orig.} & \textbf{\begin{tabular}[c]{@{}c@{}}Rule- \\ Based\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}LLM\\ Rewrite\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}} LLM- \\ Assisted \\ Rule- \\ Based\end{tabular}} \\
    
    \toprule
    
    ALL & 64.56 & \textbf{64.80} & 63.54 & \textbf{63.44} & 65.04 & \textbf{65.07} & \textbf{64.19} & \textbf{63.28} & 64.84 & \textbf{64.63} & 63.24 & \textbf{63.09} \cr
    \midrule
    Setting & 90.15 & 88.66 & 86.69 & 86.13 & 89.61 & 88.40 & 88.54 & 84.06 & 90.18 & 88.88 & 86.61 & 84.46 \cr
    Character & 84.12 & 85.18 & \textbf{83.09} & 82.98 & 85.02 & \textbf{87.24} & 81.95 & 83.75 & 84.65 & 84.41 & 80.16 & 84.07 \cr
    Action & 74.38 & 74.44 & 72.66 & \textbf{73.01} & 74.59 & 74.29 & \textbf{73.92} & \textbf{73.19} & \textbf{76.11} & \textbf{75.67} & \textbf{74.58} & \textbf{73.22} \cr
    Outcome Res. & 57.83 & 56.79 & 55.06 & 58.03 & 56.57 & 54.52 & 55.36 & 54.91 & 56.71 & 56.91 & 56.88 & 57.57 \cr
    Feeling & 48.74 & 46.28 & 45.37 & 43.45 & 48.48 & 47.51 & 46.52 & 44.68 & 50.05 & 47.21 & 45.61 & 44.38 \cr
    Causal Rel. & 54.53 & 56.53 & 56.44 & 55.19 & 55.90 & \textbf{57.57} & 56.67 & 55.50 & 53.42 & 55.65 & 54.68 & 54.77 \cr
    Prediction & 38.25 & 38.20 & 36.44 & 38.92 & 39.92 & 36.38 & 37.20 & 36.64 & 37.46 & 32.74 & 32.23 & 33.10\cr
    \bottomrule
    \end{tabular}
    }
    \caption{\label{t5-rouge-full}ROUGE-L F1 scores for the T5 model fine-tuned on the ruled-based gender augmented \texttt{FairytaleQA}  dataset (l.h.s.) and 50\% of original + 50\% of rule-based gender augmented \texttt{FairytaleQA}  dataset (center), and full original + full rule-based gender augmented \texttt{FairytaleQA}  dataset (r.h.s.) and tested on the rule-based gender augmentation, LLM gender augmentation, and LLM assisted rule based gender augmentation test dataset. Bold values indicate a statistically significant increase to the 95\% confidence compared to the results in Table~\ref{t5-rouge-original}.}
    
\end{table*}

==> extra/t5_summary.tex <==
\begin{table}[h]
\centering
\footnotesize
\scalebox{0.80}{
\begin{tabular}{lcccc}
\toprule

\textbf{Training Set} & \textbf{Original} & \textbf{\begin{tabular}[c]{@{}c@{}}Rule-\\ Based\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}LLM\\ Rewrite\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}} LLM-Assisted \\ Rule-Based\end{tabular}}\\
\midrule


Original &  65.29 & 64.38 & 63.53 & 62.66\\
Augmented & 64.56 & 64.8 & 63.54 & 63.44\\
1/2 Orig. +1/2 Aug. & 65.04 & 65.07 & 64.19 & 63.28\\
Orig. + Aug.  & 64.84 & 64.63 &  63.24 & 63.02\\

\bottomrule
\end{tabular}
}
\caption{\label{simplified-full-results-T5} ROUGE-L F1 scores for the T5 model fine-tuned on different training sets augmented using each CDA approach.}
\end{table}

